DataMaestro: A Versatile and Efficient Data Streaming Engine Bringing Decoupled Memory Access To Dataflow Accelerators

Deep Neural Networks (DNNs) have achieved remarkable success across various intelligent tasks but encounter performance and energy challenges in inference execution due to data movement bottlenecks. We introduce DataMaestro, a versatile and efficient data streaming unit that brings the decoupled access/execute architecture to DNN dataflow accelerators to address this issue. DataMaestro supports flexible and programmable access patterns to accommodate diverse workload types and dataflows, incorporates fine-grained prefetch and addressing mode switching to mitigate bank conflicts, and enables customizable on-the-fly data manipulation to reduce memory footprints and access counts. We integrate five DataMaestros with a Tensor Core-like GeMM accelerator and a Quantization accelerator into a RISC-V host system for evaluation. The FPGA prototype and VLSI synthesis results demonstrate that DataMaestro helps the GeMM core achieve nearly 100% utilization, which is 1.05-21.39x better than state-of-the-art solutions, while minimizing area and energy consumption to merely 6.43% and 15.06% of the total system.

==> outline.tex <==
\section{Theme (To be removed)}

\mv{All experiments are very heavily tuned to Gemm and matmul now. With only a single accelerator type. In this case, we have to tune down the generality of the title and the introduction. Our experiments are only in a very narrow domain.}
\begin{itemize}
    \item NN is popular. The AI workload is regular and can be represented as loops. The regularity can be utilized to parallel execute. A lot of domain specific dataflow accelerators come up, such as, BitWave \cite{shi2024bitwave}, Diana\cite{pouya2023diana}, ..
    \item However, these accelerators highly focus on the PE array versatility, such as, scale in number of PE arrays, dynamic dataflow, support of diversified data type and accuracy, data reuse and stationary. However, as the scale of PE continues to increase and data reuse and stationary had already been highly exploited before, finally the data transfer between memory module and PE array become the bottleneck, and how effective data can be provided to the PE arrays dominates the utilization of the whole system. 
    \item Compared to the general workloads, the AI workload applies similar and repetitive operations to massive data (tensors). As such, the access pattern is fixed, like linear, strided, stencil, etc and conditional branches for memory accesses are rare. These characteristics enable decoupled access and computation, in which the main idea is hardware loops with affine access patterns to accelerate the data movement process by offloading the computation of address from the processing units and deterministic data prefetch to hide the memory access latency. SSR \cite{schuiki2020stream} proposes an efficient load-store unit and leverages two specific registers for hardware data prefetch, showing $xxx\%$ improvement in matrix-multiplication workload. However, the SSR is tightly coupled to the CPU pipeline and only has 64-bit data port bandwidth, limiting its actual usage for big accelerator arrays to process data in larger scale. 
    \item research gap: each dataflow accelerator has some kind of data streaming unit to address the data movement issue between the PE array and memory~\cite{talpes2020compute, shi2024bitwave}. However, they 1) either become a dedicated hardware block tightly coupled to a specific accelerator, featuring fixed access pattern and bandwidth so that it is difficult to be used by accelerators optimized for different workload. or 2) show drawbacks in dealing with bank conflict, resulting in overall lower system efficiency (low utilization, Gemmini \cite{genc2021gemmini} example), 3) 
    need extra memory access for data re-arrangement operations (dedicated permute/transpose unit, no pipelined architecture \cite{norrie2020google}, data agin/reshuffle buffer \cite{talpes2020compute, pouya2023diana}). Gemmini \cite{genc2021gemmini} has fixed two-dimensional hardware loop and address generation patterns, killing possibilities for any data layout optimization and more complex data access pattern, such as implicit im2col for convolution layers. 
    %(Note: The limitation is not only coming from streamer architecture, but also memory architecture. The mixed wide-narrow memory system helps us to achieve im2col on-the-fly) 
    Moreover, as there is no data buffer mechanism between the on-chip SRAM and PE array to hide the memory access cycles and improper data layout, the temporal utilization of Gemmini can be as low as $10\%$ because of bank conflicts, inefficient data preprocess architecture (transpose unit, im2col unit etc) \cite{gonzalez202116mm}. 
    
    \cite{schneider2024energy} present data conductors that help the PE array fetch sparse data. However, due to the lack of a hardware loop controller, it needs one instruction to fetch data once, increasing the instruction number and execution overhead.
    
    BitWave~\cite{shi2024bitwave} is equipped with efficient and flexible data fetchers and dispatchers for both input and weight tensors, achieving dynamic dataflow to boost spatial utilization. However, the data fetchers and dispatchers are highly coupled to the specific workload and accelerator data path, limiting its reusability to different workloads or accelerator designs.
    
    \item our contribution: SoTA comparison in Table \ref{tab:sota}
    
    1) versatile data streamer generator, called \streamername, featuring design-time and runtime configurability, granularity-tunable prefetch to eliminate the bank conflict in smaller scale and utilize the on-chip SRAM bandwidth as much as possible. \mv{[should make it more clear that this is reuable across many accelerator (types) and across differend operands of an accelerator (inputs and outputs)]}
    
    2) datapath extension for data manipulation on the fly, such as transposer, broadcaster, implicit im2col on the fly 
    
    3) our case study with a GeMM accelerator shows the versatility and efficiency of the \streamername. Experimental result shows our \streamername helps the PE array achieve $xxxx$ utilization. FPGA prototype shows \streamername only occupies $xxx$ area/energy consumption of the total system.
\end{itemize}


% 3 figures: loop representation figure, \streamername main figure, GeMMX system figure (with 5 streamers highlighted and memory hierarchy)

